New Rewriter Features in FGL

FGL is a successor to GL, a proof procedure for ACL2 that allows complicated finitary conjectures to be translated into efficient Boolean function representations and proved using SAT solvers. A primary focus of FGL is to allow greater programmability using rewrite rules. While the FGL rewriter is modeled on ACL2's rewriter, we have added several features in order to make rewrite rules more powerful. A particular focus is to make it more convenient for rewrite rules to use information from the syntactic domain, allowing them to replace built-in primitives and meta rules in many cases. Since it is easier to write, maintain, and prove the soundness of rewrite rules than to do the same for rules programmed at the syntactic level, these features help make it feasible for users to precisely program the behavior or the rewriter. We describe the new features that FGL's rewriter implements, discuss the solutions to some technical problems that we encountered in their implementation, and assess the feasibility of adding these features to the ACL2 rewriter.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{G. Passmore, R. Gamboa (Eds.): ACL2 Workshop 2020\\
EPTCS 327, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.327.3}{10.4204/EPTCS.327.3}}

